FINN: A Framework for Fast, Scalable Binarized Neural Network Inference

Research has shown that convolutional neural networks contain significant redundancy, and high classification accuracy can be obtained even when weights and activations are reduced from floating point to binary values. In this paper, we present FINN, a framework for building fast and flexible FPGA accelerators using a flexible heterogeneous streaming architecture. By utilizing a novel set of optimizations that enable efficient mapping of binarized neural networks to hardware, we implement fully connected, convolutional and pooling layers, with per-layer compute resources being tailored to user-provided throughput requirements. On a ZC706 embedded FPGA platform drawing less than 25 W total system power, we demonstrate up to 12.3 million image classifications per second with 0.31 {\mu}s latency on the MNIST dataset with 95.8% accuracy, and 21906 image classifications per second with 283 {\mu}s latency on the CIFAR-10 and SVHN datasets with respectively 80.1% and 94.9% accuracy. To the best of our knowledge, ours are the fastest classification rates reported to date on these benchmarks.

==> content/5-performance_expl.tex <==
%\section{Performance exploration}
%\label{sec:performanceexpl}




==> tables/cifar10.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c | c c }
\toprule
$Layer \#$ & $Layer Type$ & $Type_{in}$ & $W_{in}$ & $H_{in}$ & $Ch_{in}$ & $Type_{out}$ & $W_{out}$ & $H_{out}$ & $Ch_{out}$  & $Kernel$ & $PoolDim$ & $P$ & $S$\\
\midrule
1  & Convolutional    & 8-bit  & 32 & 32  & 3   & Binary & 30 & 30  & 64  & 3 & - & 64  & 3 \\
2  & Convolutional    & Binary & 30 & 30  & 64  & Binary & 28 & 28  & 64  & 3 & - & 64  & 64 \\
3  & Max pooling      & Binary & 28 & 28  & 64  & Binary & 14 & 14  & 64  & - & 2 & -   & - \\
4  & Convolutional    & Binary & 14 & 14  & 64  & Binary & 12 & 12  & 128 & 3 & - & 32  & 64 \\
5  & Convolutional    & Binary & 12 & 12  & 128 & Binary & 10 & 10  & 128 & 3 & - & 32  & 64 \\
6  & Max pooling      & Binary & 10 & 10  & 128 & Binary & 5  & 5   & 128 & - & 2 & -   & - \\
7  & Convolutional    & Binary & 5  & 5   & 128 & Binary & 3  & 3   & 256 & 3 & - & 8   & 64 \\
8  & Convolutional    & Binary & 3  & 3   & 256 & Binary & 1  & 1   & 256 & 3 & - & 2   & 64 \\
9  & Fully Connected  & Binary & -  & 256 & -   & Binary & -  & 512 & -   & - & - & 1   & 16 \\
10 & Fully Connected  & Binary & -  & 512 & -   & Binary & -  & 512 & -   & - & - & 1   & 32 \\
11 & Fully Connected* & Binary & -  & 512 & -   & 16-bit & -  & 10  & -   & - & - & 4   & 1 \\
\midrule[.5pt]
\multicolumn{12}{l}{\textsuperscript{*}\footnotesize{Layer with no activation}}
\end{tabular}
}

==> tables/convmnist.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c | c c }
\toprule
$Layer \#$ & $Layer Type$ & $Type_{in}$ & $W_{in}$ & $H_{in}$ & $Ch_{in}$ & $Type_{out}$ & $W_{out}$ & $H_{out}$ & $Ch_{out}$  & $Kernel$ & $PoolDim$ & $P$ & $S$\\
\midrule
1 & Convolutional    & Binary & 28 & 28  & 1  & Binary & 25 & 25  & 8  & 4 & - & 8   & 16 \\
2 & Max pooling      & Binary & 25 & 25  & 8  & Binary & 12 & 12  & 8  & - & 2 & -   & - \\
3 & Convolutional    & Binary & 12 & 12  & 8  & Binary & 9  & 9   & 16 & 4 & - & 16  & 8 \\
4 & Max Pooling      & Binary & 9  & 9   & 16 & Binary & 4  & 4   & 16 & - & 2 & -   & - \\
5 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 256 & -  & - & - & 64  & 16 \\
6 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 10  & -  & - & - & 64  & 64 \\
\end{tabular}
}

==> tables/fcmnist.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c | c c }
\toprule
$Layer \#$ & $Layer Type$ & $Type_{in}$ & $W_{in}$ & $H_{in}$ & $Ch_{in}$ & $Type_{out}$ & $W_{out}$ & $H_{out}$ & $Ch_{out}$  & $Kernel$ & $PoolDim$ & $P$ & $S$\\
\midrule
1 & Fully Connected  & Binary & -  & 784 & -  & Binary & -  & 256  & -  & - & - & 256 & 64 \\
2 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 256  & -  & - & - & 64  & 64 \\
3 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 256  & -  & - & - & 64  & 64 \\
4 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 10        & -  & - & - & 16  & 10 \\
\midrule
1 & Fully Connected  & Binary & -  & 784      & -  & Binary & -  & 512  & -  & - & - & 256 & 64 \\
2 & Fully Connected  & Binary & -  & 512 & -  & Binary & -  & 512  & -  & - & - & 128  & 64 \\
3 & Fully Connected  & Binary & -  & 512 & -  & Binary & -  & 512  & -  & - & - & 128  & 64 \\
4 & Fully Connected  & Binary & -  & 512 & -  & Binary & -  & 10        & -  & - & - & 16  & 10 \\
\midrule
1 & Fully Connected  & Binary & -  & 784    & -  & Binary & -  & 1024  & -  & - & - & 128 & 64 \\
2 & Fully Connected  & Binary & -  & 1024   & -  & Binary & -  & 1024  & -  & - & - & 128 & 64 \\
3 & Fully Connected  & Binary & -  & 1024   & -  & Binary & -  & 1024  & -  & - & - & 128 & 64 \\
4 & Fully Connected  & Binary & -  & 1024   & -  & Binary & -  & 10    & -  & - & - & 16  & 10 \\
\midrule[.5pt]
%\multicolumn{12}{l}{\textsuperscript{*}\footnotesize{The same network architecture has been implemented with several number of neurons (1024, 512, 256)}}\\
\multicolumn{12}{l}{\footnotesize{$Type_{in}$-$Type_{out}$: datatype of input/output feature map}}\\
\multicolumn{12}{l}{\footnotesize{$W_{in}$-$W_{out}$: width of input/output feature map}}\\
\multicolumn{12}{l}{\footnotesize{$H_{in}$-$H_{out}$: height of input/output feature map}}\\
\multicolumn{12}{l}{\footnotesize{$Ch_{in}$-$Ch_{out}$: input/output feature map channels}} \\
\multicolumn{12}{l}{\footnotesize{$P$-$S$: number of PEs and number of SIMD lanes per PE}}
\end{tabular}
}

==> tables/implementation.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c c c c c c c c c c c}
\toprule
\multirow{2}{*}{$Network$} & \multirow{2}{*}{$Accuracy$} & $Latency$  & \multirow{2}{*}{$FPS$}& \multirow{2}{*}{$GOp/s$} & $power^a $ & $power$ ${eff.}^a$ & $power^b $ & $power$ ${eff.}^b$ & \multirow{2}{*}{$BRAMs$} & \multirow{2}{*}{$FF$} & \multirow{2}{*}{$LUT$} \\
 & & $[\mu s]$ & & & $[W]$ & $[Gop/s/W]$ & $[W]$ & $[Gop/s/W]$ & & & \\
\midrule
FCMNIST-256         & 95.75\% & 0.31 & 12.361 M & 8265  & 21.2  & 389.88 &  7.3 & 1132 & 130.5 & 96833 & 112408 \\
FCMNIST-512         & 97.52\% & 0.61 & 6.238 M  & 11613 & 28.5  & 407.47 & 11.3 & 1028 & 516.5 & 104614 & 123208 \\
FCMNIST-1024        & 98.28\% & 2.44 & 1.561 M  & 9086  & 23.4  & 391.62 &  8.8 & 1032 & 398   & 80055 & 92754 \\
%Convolutional MNIST & 95.13\% & 12  & 117159   &  146  & 9.4   & 15.53  &  0.9 & 162  & 102  & 21730 & 20244\\
Cifar10small        & 78.52\% & 283 & 21906    & 2465   & 11.7  & 210.72 &  3.6 & 685 & 192  & 59763 & 54509 \\
\midrule
FCMNIST-512*        & 97.52\% & 3   & 2.196 M  & 4088  & 14.6  & 280.01 &  4.4 & 929  & 386.5 & 80402 & 94250 \\
FCMNIST-1024*       & 98.28\% & 5   & 459 k    & 2676  & 12.6  & 212.35 &  3.3 & 811  & 397  & 80038 & 93607 \\
\midrule[.5pt]
\multicolumn{10}{l}{\textsuperscript{*}\footnotesize{Unoptimized hardware implementations}} \\
\multicolumn{10}{l}{\textsuperscript{a}\footnotesize{Board power}} \\
\multicolumn{10}{l}{\textsuperscript{b}\footnotesize{PL power}} 
\end{tabular}
}
